Dynamic Markers: UAV landing proof of concept

In this paper, we introduce a dynamic fiducial marker which can change its appearance according to the spatiotemporal requirements of the visual perception task of a mobile robot using a camera as the sensor. We present a control scheme to dynamically change the appearance of the marker in order to increase the range of detection and to assure a better accuracy on the close range. The marker control takes into account the camera to marker distance (which influences the scale of the marker in image coordinates) to select which fiducial markers to display. Hence, we realize a tight coupling between the visual pose control of the mobile robot and the appearance of the dynamic fiducial marker. Additionally, we discuss the practical implications of time delays due to processing time and communication delays between the robot and the marker. Finally, we propose a real-time dynamic marker visual servoing control scheme for quadcopter landing and evaluate the performance on a real-world example.

==> img/marker_displacement.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=6cm,
height=1.8cm,
at={(0.809in,0.513in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
xmin=-1,
xmax=1,
xlabel={\footnotesize x Coordinate (m)},
xmajorgrids,
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
ymin=0,
ymax=0.03,
ylabel={\footnotesize Absolute Error (m)},
ymajorgrids,
axis background/.style={fill=white},
legend style={at={(0.2,0.97)},anchor=north west,legend cell align=left,align=left,fill=white},
every x tick label/.append style={font=\footnotesize},
every y tick label/.append style={font=\footnotesize}
]

\addplot [color=blue,solid,line width=1.0pt]
  table[row sep=crcr]{%
-1.002	0.0298023562490004\\
-0.992	0.0297086046730061\\
-0.982	0.0296054662462277\\
-0.972	0.0294935146928614\\
-0.962	0.0293733237371036\\
-0.952	0.0292454671031507\\
-0.942	0.0291105185151992\\
-0.932	0.0289690516974453\\
-0.922	0.0288216403740855\\
-0.912	0.0286688582693161\\
-0.902	0.0285112791073336\\
-0.892	0.0283420873442159\\
-0.882	0.02815605163166\\
-0.872	0.0279561219872907\\
-0.862	0.0277452484287325\\
-0.852	0.0275263809736102\\
-0.842	0.0273024696395484\\
-0.832	0.0270764644441719\\
-0.822	0.0268513154051052\\
-0.812	0.0266299725399731\\
-0.802	0.0264153858664002\\
-0.792	0.0262014795834111\\
-0.782	0.0259818366661935\\
-0.772	0.0257588952966166\\
-0.762	0.0255350936565497\\
-0.752	0.0253128699278623\\
-0.742	0.0250946622924234\\
-0.732	0.0248829089321026\\
-0.722	0.024680048028769\\
-0.712	0.024488517764292\\
-0.702	0.0243108208035172\\
-0.692	0.0241550615120531\\
-0.682	0.0240205679939052\\
-0.672	0.0239001446749407\\
-0.662	0.023786595981027\\
-0.652	0.0236727263380314\\
-0.642	0.0235513401718214\\
-0.632	0.0234152419082642\\
-0.622	0.0232572359732272\\
-0.612	0.0230701267925777\\
-0.602	0.0228439843105426\\
-0.592	0.0224903603419837\\
-0.582	0.0219917528270675\\
-0.572	0.0213784048713788\\
-0.562	0.0206805595805026\\
-0.552	0.0199284600600238\\
-0.542	0.0191523494155273\\
-0.532	0.0183824707525979\\
-0.522	0.0176490671768206\\
-0.512	0.0169823817937803\\
-0.502	0.0164121556946454\\
-0.492	0.0159027422335104\\
-0.482	0.0154151890000672\\
-0.472	0.0149467537263117\\
-0.462	0.0144946941442395\\
-0.452	0.0140562679858464\\
-0.442	0.0136287329831283\\
-0.432	0.0132093468680809\\
-0.422	0.0127953673727\\
-0.412	0.0123840522289813\\
-0.402	0.0119726465184037\\
-0.392	0.0115581224634506\\
-0.382	0.011141891315152\\
-0.372	0.0107271971764901\\
-0.362	0.0103172841504473\\
-0.352	0.00991539634000587\\
-0.342	0.00952477784814812\\
-0.332	0.00914867277785636\\
-0.322	0.00879032523211289\\
-0.312	0.00845297931390003\\
-0.302	0.00813987912620007\\
-0.292	0.00784419079689255\\
-0.282	0.00755742797406302\\
-0.272	0.00728035604100287\\
-0.262	0.00701374038100348\\
-0.252	0.00675834637735621\\
-0.242	0.00651493941335246\\
-0.232	0.00628428487228359\\
-0.222	0.00606714813744099\\
-0.212	0.00586429459211603\\
-0.202	0.0056764896196001\\
-0.192	0.00549102520264199\\
-0.182	0.00529873989248113\\
-0.172	0.00510571892514477\\
-0.162	0.0049180475366602\\
-0.152	0.00474181096305467\\
-0.142	0.00458309444035547\\
-0.132	0.00444798320458986\\
-0.122	0.00434256249178512\\
-0.112	0.00427291753796851\\
-0.102	0.00424513357916732\\
-0.092	0.00427305677269237\\
-0.082	0.00436552834983537\\
-0.072	0.00451454245495953\\
-0.0619999999999999	0.00471197373426872\\
-0.0519999999999999	0.00494969683396678\\
-0.042	0.00521958640025757\\
-0.032	0.00551351707934494\\
-0.022	0.00582336351743275\\
-0.012	0.00614100036072485\\
-0.002	0.00645830225542508\\
0.00800000000000001	0.00679405359103616\\
0.018	0.00719375360611804\\
0.0279999999999999	0.00764750650673852\\
0.0379999999999999	0.00814371147021671\\
0.0479999999999999	0.00867076767387165\\
0.0579999999999999	0.00921707429502242\\
0.0679999999999999	0.0097710305109881\\
0.078	0.0103210354990878\\
0.088	0.0108610075077738\\
0.098	0.0114157059044368\\
0.108	0.0119873436658898\\
0.118	0.0125729753381758\\
0.128	0.013169655467338\\
0.138	0.0137744385994194\\
0.148	0.0143843792804634\\
0.158	0.0149965320565128\\
0.168	0.015607951473611\\
0.178	0.016215692077801\\
0.188	0.0168180384308074\\
0.198	0.0174495077211001\\
0.208	0.0181151920995619\\
0.218	0.0187991132994771\\
0.228	0.0194852930541304\\
0.238	0.0201577530968064\\
0.248	0.0208005151607897\\
0.258	0.0213976009793648\\
0.268	0.0219330322858163\\
0.278	0.0223908308134289\\
0.288	0.0227601796412163\\
0.298	0.0230801058615703\\
0.308	0.0233671436329461\\
0.318	0.0236275480899895\\
0.328	0.0238675743673464\\
0.338	0.0240934775996627\\
0.348	0.0243115129215841\\
0.358	0.0245279354677566\\
0.368	0.0247490003728261\\
0.378	0.0249809627714385\\
0.388	0.0252291498882536\\
0.398	0.0254902682563006\\
0.408	0.0257594710714481\\
0.418	0.0260323970904724\\
0.428	0.0263046850701498\\
0.438	0.0265719737672568\\
0.448	0.0268299019385699\\
0.458	0.0270741083408654\\
0.468	0.0273002317309197\\
0.478	0.0275039108655092\\
0.488	0.02768155543567\\
0.498	0.0278542327807\\
0.508	0.0280298710155892\\
0.518	0.0282040578636003\\
0.528	0.0283723810479955\\
0.538	0.0285304282920375\\
0.548	0.0286737873189886\\
0.558	0.0287980458521115\\
0.568	0.0288987916146684\\
0.578	0.0289716123299221\\
0.588	0.0290120957211348\\
0.598	0.0290148599056791\\
0.608	0.0289703246895836\\
0.618	0.0288828335737184\\
0.628	0.0287596098035377\\
0.638	0.0286078766244957\\
0.648	0.0284348572820468\\
0.658	0.028247775021645\\
0.668	0.0280538530887447\\
0.678	0.0278603147288\\
0.688	0.0276165967701611\\
0.698	0.027284295581156\\
0.708	0.0268888737172058\\
0.718	0.0264557937337314\\
0.728	0.026010518186154\\
0.738	0.0255785096298945\\
0.748	0.0251852306203739\\
0.758	0.0248561437130133\\
0.768	0.0246167114632337\\
0.778	0.0244923964264561\\
0.788	0.0244910226979586\\
0.798	0.0245496873759822\\
0.808	0.0246498518096321\\
0.818	0.0247798259269007\\
0.828	0.0249279196557808\\
0.838	0.0250824429242649\\
0.848	0.0252317056603457\\
0.858	0.0253640177920159\\
0.868	0.0254676892472679\\
0.878	0.0255310299540946\\
0.888	0.0255381211109066\\
0.898	0.0254176303317021\\
0.908	0.0251579200856761\\
0.918	0.0247724280225794\\
0.928	0.0242745917921623\\
0.938	0.0236778490441755\\
0.948	0.0229956374283694\\
0.958	0.0222413945944947\\
0.968	0.0214285581923018\\
0.978	0.0205705658715413\\
};
\addlegendentry{\footnotesize Aruco 88};

\addplot [color=red,solid,line width=1.0pt]
  table[row sep=crcr]{%
-1.099	0.0176733424669995\\
-1.089	0.0173400539070047\\
-1.079	0.0170151322936095\\
-1.069	0.0166991406899197\\
-1.059	0.0163926421590411\\
-1.049	0.0160961997640797\\
-1.039	0.0158103765681412\\
-1.029	0.0155357356343316\\
-1.019	0.0152728400257567\\
-1.009	0.0150222528055224\\
-0.999	0.0147845535289352\\
-0.989	0.0145615820301046\\
-0.979	0.0143523664040223\\
-0.969	0.0141541508278222\\
-0.959	0.0139641794786385\\
-0.949	0.0137796965336053\\
-0.939	0.0135979461698566\\
-0.929	0.0134161725645267\\
-0.919	0.0132316198947495\\
-0.909	0.0130415323376591\\
-0.899	0.0128431321399012\\
-0.889	0.0126349472034141\\
-0.879	0.0124194158343364\\
-0.869	0.0121995682660611\\
-0.859	0.0119784347319815\\
-0.849	0.0117590454654905\\
-0.839	0.0115444306999813\\
-0.829	0.0113376206688468\\
-0.819	0.0111416456054802\\
-0.809	0.0109595357432746\\
-0.799	0.0107934042634347\\
-0.789	0.0106366054546287\\
-0.779	0.0104866726544657\\
-0.769	0.0103429834065934\\
-0.759	0.0102049152546599\\
-0.749	0.010071845742313\\
-0.739	0.00994315241320058\\
-0.729	0.00981821281097063\\
-0.719	0.00969640447927103\\
-0.709	0.00957710496174968\\
-0.699	0.00946004156970436\\
-0.689	0.00934772122630833\\
-0.679	0.00924000351478362\\
-0.669	0.00913594157703553\\
-0.659	0.00903458855496934\\
-0.649	0.00893499759049032\\
-0.639	0.00883622182550376\\
-0.629	0.00873731440191494\\
-0.619	0.00863732846162914\\
-0.609	0.00853531714655166\\
-0.599	0.00843028484770663\\
-0.589	0.0083203333226229\\
-0.579	0.00820618266827047\\
-0.569	0.00808962517113961\\
-0.559	0.00797245311772061\\
-0.549	0.00785645879450375\\
-0.539	0.0077434344879793\\
-0.529	0.00763517248463755\\
-0.519	0.00753346507096878\\
-0.509	0.00744010453346326\\
-0.499	0.0073560638843753\\
-0.489	0.0072773577996254\\
-0.479	0.00720275649163018\\
-0.469	0.00713175367313628\\
-0.459	0.00706384305689029\\
-0.449	0.00699851835563884\\
-0.439	0.00693527328212855\\
-0.429	0.00687360154910602\\
-0.419	0.00681299686931789\\
-0.409	0.00675295295551076\\
-0.399	0.0066929397979377\\
-0.389	0.00663257711801926\\
-0.379	0.00657229927912129\\
-0.369	0.00651265746870285\\
-0.359	0.00645420287422305\\
-0.349	0.00639748668314096\\
-0.339	0.00634306008291569\\
-0.329	0.0062914742610063\\
-0.319	0.0062432804048719\\
-0.309	0.00619902970197157\\
-0.299	0.00615931166377986\\
-0.289	0.00612477130290396\\
-0.279	0.00609450293136827\\
-0.269	0.00606724409408263\\
-0.259	0.00604173233595684\\
-0.249	0.00601670520190072\\
-0.239	0.0059909002368241\\
-0.229	0.0059630549856368\\
-0.219	0.00593190699324862\\
-0.209	0.0058961938045694\\
-0.199	0.00585432735819359\\
-0.189	0.00580096424456273\\
-0.179	0.00573651346829786\\
-0.169	0.00566346306999593\\
-0.159	0.00558430109025385\\
-0.149	0.00550151556966854\\
-0.139	0.00541759454883695\\
-0.129	0.00533502606835598\\
-0.119	0.00525629816882256\\
-0.109	0.00518389889083363\\
-0.099	0.00512005671971788\\
-0.089	0.00506217295958095\\
-0.079	0.00500808977321543\\
-0.069	0.00495677497228944\\
-0.0589999999999999	0.00490719636847115\\
-0.0489999999999999	0.00485832177342867\\
-0.0389999999999999	0.00480911899883017\\
-0.0289999999999999	0.00475855585634378\\
-0.0189999999999999	0.00470560015763763\\
-0.0089999999999999	0.00464921971437989\\
0.00100000000000011	0.00458835169329457\\
0.0110000000000001	0.00451913821794994\\
0.0210000000000001	0.00444145515328316\\
0.031	0.00435818972569189\\
0.041	0.00427222916157382\\
0.051	0.00418646068732662\\
0.0610000000000001	0.00410377152934797\\
0.0710000000000001	0.00402704891403553\\
0.0810000000000001	0.00395918006778699\\
0.0910000000000001	0.00390305221700002\\
0.101	0.00385698949576955\\
0.111	0.00381653773751348\\
0.121	0.00378041671761396\\
0.131	0.00374734621145312\\
0.141	0.0037160459944131\\
0.151	0.00368523584187603\\
0.161	0.00365363552922405\\
0.171	0.00361996483183929\\
0.181	0.00358294352510389\\
0.191	0.00354129138439999\\
0.201	0.00349473947342969\\
0.211	0.00344425536732422\\
0.221	0.0033904136086094\\
0.231	0.00333378873981107\\
0.241	0.00327495530345503\\
0.251	0.00321448784206712\\
0.261	0.00315296089817315\\
0.271	0.00309094901429895\\
0.281	0.00302902673297035\\
0.291	0.00296720271322595\\
0.301	0.00290273790887199\\
0.311	0.00283584979902316\\
0.321	0.00276733082541512\\
0.331	0.0026979734297835\\
0.341	0.00262857005386396\\
0.351	0.00255991313939213\\
0.361	0.00249279512810367\\
0.371	0.00242800846173421\\
0.381	0.00236634558201942\\
0.391	0.00230714094770277\\
0.401	0.00224315034874605\\
0.411	0.00217552587301687\\
0.421	0.00210695661872822\\
0.431	0.00204013168409311\\
0.441	0.00197774016732451\\
0.451	0.00192247116663542\\
0.461	0.00187701378023883\\
0.471	0.00184405710634774\\
0.481	0.00182629024317514\\
0.491	0.00182469572942123\\
0.501	0.00183024789021362\\
0.511	0.00184015875667482\\
0.521	0.00185318298432802\\
0.531	0.00186807522869641\\
0.541	0.0018835901453032\\
0.551	0.0018984823896716\\
0.561	0.00191150661732479\\
0.571	0.00192141748378599\\
0.581	0.00192696964457839\\
0.591	0.00192713309057829\\
0.601	0.00192279086967554\\
0.611	0.00191505038893586\\
0.621	0.00190489665121052\\
0.631	0.00189331465935083\\
0.641	0.00188128941620805\\
0.651	0.00186980592463349\\
0.661	0.00185984918747841\\
0.671	0.00185240420759411\\
0.681	0.00184845598783188\\
0.691	0.00185341164780703\\
0.701	0.00188431881495603\\
0.711	0.00193929804045856\\
0.721	0.00201437216596724\\
0.731	0.00210556403313465\\
0.741	0.00220889648361339\\
0.751	0.00232039235905607\\
0.761	0.00243607450111529\\
0.771	0.00255196575144365\\
0.781	0.00266408895169373\\
0.791	0.00277294665726572\\
0.801	0.0028864434595353\\
0.811	0.0030057427832235\\
0.821	0.00313176069242506\\
0.831	0.00326541325123472\\
0.841	0.00340761652374723\\
0.851	0.00355928657405733\\
0.861	0.00372133946625976\\
0.871	0.00389469126444926\\
0.881	0.00408025803272057\\
0.891	0.00428088772840623\\
0.901	0.00450802196374982\\
0.911	0.00476178495615156\\
0.921	0.00504025060629857\\
0.931	0.00534149281487798\\
0.941	0.00566358548257691\\
0.951	0.00600460251008247\\
0.961	0.0063626177980818\\
0.971	0.00673570524726202\\
0.981	0.00712193875831024\\
};
\addlegendentry{\footnotesize Whycon};
\legend{};

\end{axis}
\end{tikzpicture}%
